Effective Few-Shot Named Entity Linking by Meta-Learning

Entity linking aims to link ambiguous mentions to their corresponding entities in a knowledge base, which is significant and fundamental for various downstream applications, e.g., knowledge base completion, question answering, and information extraction. While great efforts have been devoted to this task, most of these studies follow the assumption that large-scale labeled data is available. However, when the labeled data is insufficient for specific domains due to labor-intensive annotation work, the performance of existing algorithms will suffer an intolerable decline. In this paper, we endeavor to solve the problem of few-shot entity linking, which only requires a minimal amount of in-domain labeled data and is more practical in real situations. Specifically, we firstly propose a novel weak supervision strategy to generate non-trivial synthetic entity-mention pairs based on mention rewriting. Since the quality of the synthetic data has a critical impact on effective model training, we further design a meta-learning mechanism to assign different weights to each synthetic entity-mention pair automatically. Through this way, we can profoundly exploit rich and precious semantic information to derive a well-trained entity linking model under the few-shot setting. The experiments on real-world datasets show that the proposed method can extensively improve the state-of-the-art few-shot entity linking model and achieve impressive performance when only a small amount of labeled data is available. Moreover, we also demonstrate the outstanding ability of the model's transferability.

==> meta.tex <==
%!TEX root=../main.tex



\section*{Responses to The Meta Reviewer}


\begin{shaded}
\noindent \emph{\underline{COMMENT W1}: The paper studies the problem of mortality prediction using medical knowledge and text, using deep learning and a co-attention model. The paper presents a nice contribution, provided that some issues raised by the reviewers are carefully adressed in a revision. In particular, expanding the empirical evaluation beyond one dataset.  comparing with related work by Cao et al., and W2/W3 in review 3.}
\end{shaded}

%\vspace{.25em}

\noindent{\bf RESPONSE}: 
We would like to thank for your thoughtful reviews and encouraging comments, based on which we have improved the paper. The revised parts are highlighted in the paper and the responses to the comments are summarized below.
We have addressed all the comments raised by the three reviewers. Specifically, (1) we have  performed experiments on a new dataset; (2) we have compared our models with the work from Cao et al. (3) we have carefully corrected the W2/W3 issues. 

 
%See the detailed responses to the three reviewers. 




==> response.tex <==
%!TEX root=../main.tex

%% $Id: r2.tex 4261 2011-09-02 15:03:00Z guoliang $

%\newpage

\vspace{-0.25em}
\section*{Responses to Reviewer \#1}
\vspace{-.5em}


\begin{shaded}
\noindent \emph{\underline{COMMENT W1}: The illustration of how "concepts" are able to provide higher level knowledge of patients can be further explored. A weighted sum of words is not revealing too much of the nature of the concepts. }

\vspace{.1em}

%\noindent \emph{\underline{COMMENT D1}: }
\end{shaded}

\vspace{-.5em}

\noindent{\bf RESPONSE}: 
Thank you for your reviews. The main point of our paper is to study how to combine the concepts with texts in hospital mortality prediction. The medical notes contain the detailed information of the patients while these information of diseases or medical measures are not explicitly observed by using words in the document. With medical concepts extracted, some knowledge can be further explored beyond the medical notes. What is more, we use knowledge based information to guide the learning process of raw medical documents. The usage of concepts in our models has two main contributions: one is that the concepts have relations with medical knowledge and the importance of hospital mortality; the other is that concepts in the document can guide the learning process of raw medical documents. 



%\begin{shaded}
%\noindent \emph{\underline{COMMENT W2}:  The techniques, while integrated in a nice way, are well established each, therefore undermining novelty part to a certain degree. }
%\end{shaded}
%
%\vspace{-.5em}
%
%
%\noindent{\bf RESPONSE}: 
%
%Thanks for your comments. 
\vspace{.5em}


\begin{shaded}
\noindent \emph{\underline{COMMENT W3 and D1}: W3:There are some occasional typos. 
D1:Except for a few typos, e.g., "Section ??" on Page 11.}
\end{shaded}

\noindent{\bf RESPONSE}: 
Thank you for your checking. We have make careful corrections on the spelling and grammar mistakes issued by the reviewers. For example, we have checked the grammar with the help of the advisors and repainted some pictures such as Figure~\ref{fig:basic_word_level} and Figure~\ref{fig:atten_int}. In addition, we have changed the illustrations of the experiments in Section~\ref{sec-exp}. 


% \begin{shaded}
% \noindent \emph{\underline{COMMENT D1}:  }
% \end{shaded}

% \vspace{.1em}

% \noindent{\bf RESPONSE}:  
% Thanks for the comments. We are still working on the paper's writing after the submitting. And we make careful check on the paper's grammer according to the reviewer's comments.
\vspace{-0.25em}
\section*{Responses to Reviewer \#2}
\vspace{-.5em}

\begin{shaded}
\noindent \emph{\underline{COMMENT}: In fact, Cao et. al is highly relevant to the paper and I was expecting to see some comparison expts with the work in Cao et. al. Unofrtunately, this is not the case.}
\end{shaded}

\vspace{.1em}

\noindent{\bf RESPONSE}: 
We would like to express our gratitude for your professional questions. There are main differences between ours and Cao et.al. Firstly, Cao et.al uses an RNN based framework to solve short text classification problem which is quite different from the condition of ours. As is shown in medical note analysis in Table~\ref{table:notes_rad_desp}, the length of tokens varies a lot and cannot be taken as a short text classification problem. Secondly, Cao et.al only used one side attention which is different from ours, and we leverage the co-attention mechanism in both of the concept modeling and text modeling. Thirdly, the concepts in Cao's are different from ours. The concepts in Cao's is somehow coarse-grained while the concepts in ours are more fine-grained. For example, the ``heart attack'' will be recognized as ``disease"  while in our work, we explicitly use Metamap to recognize the concept ``heart attack".  Moreover,  Cao et.al used a word replace strategy to replace the words by the corresponding concepts which may lose information while we model concepts and notes in parallel. 

In order to compare our work with Cao's, we conduct a new dataset based on the documents and medical concepts. In our work, we take UMLS concepts as the concepts in Cao's and replace the corresponding tokens by the concepts' position and length. Besides, we have pointed out the differences in Section~\ref{model-aware-relate} and added the corresponding experimental results in Section~\ref{sec-exp}.

% \begin{shaded}
% \noindent \emph{\underline{COMMENT}:The proposed BK-DNN and the co-attention mechanism are relatively straightforward.}
% \end{shaded}

% \vspace{.1em}

% \noindent{\bf RESPONSE}:
% Thanks for your review. The aim of our paper is to explore the methods to integrate the medical knowledge into text based mortality prediction which has not been studied before. We show that in text based hospital mortality prediction, our models outperform the state-of-art methods. In our future work, more complex technologies and fine-gained features of medical knowledge will be studied.   

\begin{shaded}
\noindent \emph{\underline{COMMENT}:One major challenge in extracting from medical notes are the use of non standard abbreviation and shorthand notations. Again, this has been ignored in this paper.}
\end{shaded}

\vspace{.1em}

\noindent{\bf RESPONSE}: 
Thanks for your thoughtful review.  We agree that it is a major challenge in extracting from medical notes which contain non-standard abbreviation and shorthand notations.  However, we are aiming at solving the challenge of how to combine medical knowledge and medical notes together to predict hospital mortality. Therefore, the detailed information of how Metamap works is ignored in the paper. However, we indeed have done some surveys on concept extraction tools and come to a conclusion that Metamap is suitable for our problem settings. And we choose Metamap as our medical concept extractor because it is designed to map biomedical text to the UMLS concepts, and it is designed by medical experts and widely used both in researches and industries. 
% The followings are some detailed design information of the metamap.    
%
%The metamap  is a  medical concept tool designed for the UMLS. 
\begin{shaded}
\noindent \emph{\underline{COMMENT W1}: Only 1 dataset is used in the evaluation. This makes it difficult to conclude about the generalization of the proposed solution.}
\end{shaded}

\vspace{-.5em}

\noindent{\bf RESPONSE}: 
Thanks for your review. Medical notes are hard to access and very few datasets are publicly available due to their specialty and security issues. We have tried hard to negotiate with many health centers for suitable datasets. Unfortunately, due to the Law of Network Security, we are not allowed to get access to those medical databases. Besides, we have surveyed the open medical datasets but found that MIMIC III is the only suitable open dataset for our problem. In addition, in medical data mining, due to some issues of privacy protection, the datasets in the previous works are not open to us and some works are based only on the MIMIC III dataset. 

In order to illustrate its generalization ability of our proposed work, we test the proposed models on two subcategories of notes in MIMIC III, one comes from the test examinations and the other comes from caregivers. Both of the datasets are written by experienced experts but have different writing styles. We conducted experiments on those two datasets to show the strengths of our BK-DDN and AK-DDN. The detailed information and experimental results are described and highlighted in Section~\ref{sec-exp}. 

 


\begin{shaded}
\noindent \emph{\underline{COMMENT W2}: Too many references and the highly relevant works are not given sufficient treatment.}
\end{shaded}

\vspace{-.5em}


\noindent{\bf RESPONSE}: 
Thanks for your thoughtful review.  The task is related to many domains such as document classification, knowledge-based medical prediction, and some medical researches. Inspired by these works, we present the novel knowledge-based models.  The issue we are working on has some relations with these tasks. However, we are the first to adopt explicit concepts with medical notes in the text based hospital mortality prediction task. In order to solve this issue, we have improved the reference part based on your review.

\vspace{.5em}


\begin{shaded}
\noindent \emph{\underline{COMMENT W3}: More detailed discussions concerning the findings in Table V and Table VI. One sentence saying "the concept provide a higher level abstraction of the patients .... the overall status of the patients can be observed" is too vague and does not provide the necessary insights on what the authors are trying to convey. }
\end{shaded}
  


\vspace{.1em}

\noindent{\bf RESPONSE}: 
We would like to thank for your reviews. Saying ``the concepts provide a higher level abstraction of the patients .... the overall status of the patients can be observed", we want to show that the patients' status such as the medication, cure measurements and diagnosis can be explicitly obtained from the medical concepts. And we can take a simple example from Figure~\ref{fig:text-umls-demo}. The left is a demo of a note. However, the medical concepts are hidden in the text while using medical concepts makes the diseases and the medical procedure explicit. These can give a more straightforward and explicit view of a patient than raw texts.  Besides, we have improved the results of the weights in AK-DDN and we provide a pair based results and the results show that the attention works for the patients both die in the hospital and out of the hospital. 

We have changed the description of the importance of the concepts by table~\ref{table:case_neg_concept},~\ref{table:case_pos_concept}. From the table, we can get some descriptions of a patient in an ICU such as diseases, medical measures and so on. And the concepts can be considered as a high-level summary of a patient such as diseases and medical measurements but lack of detailed descriptive information such as the status of diseases. With attention, we can show that our model can capture the patients' status described in the Tables~\ref{table:case_pos_word},~\ref{table:case_pos_concept},~\ref{table:case_neg_word},~\ref{table:case_pos_concept}. 
\begin{shaded}
\noindent \emph{\underline{COMMENT D1}: Figure 8, the graph for Text CNN seems very strange with large fluctuations. Perhaps some explanation on what causes the large fluctuation is needed.}
\end{shaded}

\vspace{.1em}

\noindent{\bf RESPONSE}:  

Thanks for your review. We use figure 8 to show the trend of the training process. Although there are large fluctuations in Figure 8, with the steps goes on, the trend of these lines becomes smooth. We put the figure here to show that our models are more stable than Text CNN which only models in a one-side way. The large fluctuations can be caused by the limited number of samples and the variable lengths of tokens in the medical notes. In order to train the Text CNN, we extend the medical texts to construct a fix-length matrix. However, with the attention mechanism, those added values can be filtered out by the weights.    

\vspace{-0.25em}
\section*{Responses to Reviewer \#3}
\vspace{-.5em}


\begin{shaded}
\noindent \emph{\underline{COMMENT W1}:The structure of the proposed model is a bit simple although the idea of combining text and concepts is novel. Concept and text modeling in the proposed model is not very complicated. 
}
\end{shaded}

\vspace{-.5em}

\noindent{\bf RESPONSE}: 
 Thanks for your review. The BK-DDN and AK-DDN model the concepts and texts which has not been done in the previous work. To the best of our knowledge, we are the first to integrate medical knowledge with medical documents for text based hospital mortality prediction. Besides, we have provided a nice way of integrating concepts with medical texts and the experimental results show that our models outperform the state-of-art models.  



\begin{shaded}
\noindent \emph{\underline{COMMENT W2}: Some writing mistakes should be corrected in the paper. For example, the softmax function. Besides, the examples illustrated in table 1 are conflict where the concept indexed by C0392360 are not medical concepts. In table VI, the meanings of concepts are not illustrated clearly.The exact meanings of table VI are not illustrated in the paper, which makes the readers hard to understand. }
\end{shaded}

\vspace{-.5em}


\noindent{\bf RESPONSE}: 
Thanks for your review. After we submitted the paper, we have further improved the paper's writing and make careful grammar checks. We have corrected the writing mistakes posed by the reviewers and made some changes in the Section~\ref{word_concept_analysis}. And we have listed the descriptions of the concepts we used. 



\begin{shaded}
\noindent \emph{\underline{COMMENT D3}:However, there are many writing mistakes which need to be checked and corrected in the revision. And the results of the baseline called concept CNN is not listed in the evaluation table which need to be added. }
\end{shaded}

\vspace{.1em}

\noindent{\bf RESPONSE}:  
Thanks for your review. We have made corrections based on your review. We have added the results of Concept CNN posed by the reviewer and made careful corrections on the paper's writings with the help of the advisors.
Besides, we have repainted some pictures in the paper such as Figure~\ref{fig:basic_word_level} and fixed some painting errors in Figures~\ref{fig:atten_int}. And the illustrations of the results are updated in Section~\ref{sec-exp}. 






==> sec8-related_work.tex <==
\section{Related Work}\label{sec-related_work}
